Mating non-renormalizable quadratic polynomials

In this paper we prove the existence and uniqueness of matings of the basilica with any quadratic polynomial which lies outside of the 1/2-limb of M, is non-renormalizable, and does not have any non-repelling periodic orbits.

==> psfrag.tex <==
% Plain TeX interface to psfrag.
% David Carlisle

\input miniltx

\makeatletter

\ifx\@compatibilitytrue\@undefined
  \csname newif\expandafter\endcsname
       \csname if@compatibility\endcsname
\fi


\ifx\raisebox\@undefined
\def\raisebox#1#2{{%
  \setbox0=\hbox{#2}\def\depth{\dp0}\leavevmode\raise#1\box\z@}}
\fi

\ifx\@@underline\@undefined
\let\@@underline\underline
\def\underline{%
  \ifmmode\expandafter\@@underline\else\expandafter\underbar\fi}
\fi

\ifx\sbox\@undefined
\def\sbox#1{\setbox#1\hbox}
\fi


% psfrag loads the core graphics package, but only the extended
% graphicx interface is available from plain TeX so just intercept
% the call and ask for graphicx.
\let\savedRP\RequirePackage
\def\RequirePackage#1{%
  \let\RequirePackage\savedRP
  \ifx\includegraphics\@undefined
  \input graphicx\fi\relax}
\input psfrag.sty



\ifx\pfg@dp\@undefined
\csname newdimen\endcsname\pfg@dp
\csname newdimen\endcsname\pfg@wd
\csname newdimen\endcsname\pfg@dx
\csname newdimen\endcsname\pfg@dy
\fi

\resetatcatcode

